PR-Net: Preference Reasoning for Personalized Video Highlight Detection

Personalized video highlight detection aims to shorten a long video to interesting moments according to a user's preference, which has recently raised the community's attention. Current methods regard the user's history as holistic information to predict the user's preference but negating the inherent diversity of the user's interests, resulting in vague preference representation. In this paper, we propose a simple yet efficient preference reasoning framework (PR-Net) to explicitly take the diverse interests into account for frame-level highlight prediction. Specifically, distinct user-specific preferences for each input query frame are produced, presented as the similarity weighted sum of history highlights to the corresponding query frame. Next, distinct comprehensive preferences are formed by the user-specific preferences and a learnable generic preference for more overall highlight measurement. Lastly, the degree of highlight and non-highlight for each query frame is calculated as semantic similarity to its comprehensive and non-highlight preferences, respectively. Besides, to alleviate the ambiguity due to the incomplete annotation, a new bi-directional contrastive loss is proposed to ensure a compact and differentiable metric space. In this way, our method significantly outperforms state-of-the-art methods with a relative improvement of 12% in mean accuracy precision.

==> 2.1_Related_work_sub.tex <==
\subsection{Explainable Recommendation}
Several methods focused on incorporating knowledge graphs (KGs) into recommender systems or e-commerce systems for coupling recommendation and interpretability \cite{pecune2019model,xian2020cafe,wang2019explainable,kuang2019fashion,xian2020neural,xian2019reinforcement,cao2019unifying}. \cite{pecune2019model} proposed a conversational movie recommendation agent based on defined and annotated explanation categories. \cite{kuang2019fashion} proposed to solve the clothing matching issue in e-commerce by building a graph of similarity and training a graph convolutional network to enable the alignment. \cite{xian2020cafe,xian2020neural} proposed neural symbolic reasoning approaches which first generate user profiles and then guide a path-finding process to derive reasoning paths for recommendations. \cite{xian2019reinforcement} proposed a reinforcement learning approach and a policy-guided graph search algorithm to sample reasoning paths for recommendation. \cite{wang2019explainable} proposed to fully explore the sequential dependencies within paths (i.e., user-item connectivity) in a KG by a path recurrent network to infer the user preferences. \cite{cao2019unifying} further considered the incomplete nature of KG by jointly learning the model of recommendation and knowledge graph completion.

Some works focused on multi-hop question answering \cite{ding2019cognitive,feng2020learning}. \cite{ding2019cognitive} proposed a framework that gradually builds a cognitive graph (knowledge graph) which providing explainable reasoning paths. And \cite{feng2020learning} proposed a cooperative game approach to learn to recover reasoning chains for multi-hop question answering.

==> backup.tex <==


\begin{table}[h]
    %\scriptsize
	\centering
	\caption{Ablation Study Experiments }\label{tab:comparisons}
	\scalebox{1}{
	\begin{tabular}{c c}
        \hline
%         \multirow{2}*{backbone} &
% 		\multirow{2}*{attention strategy} &
        % \multirow{2}*{ablation target} &
		\multirow{2}*{method} &
		\multirow{2}*{mAP(\%)} \\

		~ & ~ \\
% 		\hline
% 	    baseline & - \\
	    \hline
	    SA-PR w/ residual backbone & 16.69 \\
        \hline
		SA-PR w/ ranking loss & 16.85 \\
		SA-PR w/ ce loss& 17.09 \\
		\hline
		 SA-PR w/ user-specific preference only & 17.57 \\
		 SA-PR w/ generic preference only & 16.78 \\
		\hline
		SA-PR w/ five history & 17.48 \\
		\hline
		SA-PR & \textbf{18.66} \\ 
		
	\end{tabular}}
\end{table}

\begin{table}[h]
    %\scriptsize
	\centering
	\caption{Comparison with state-of-the-art methods on the PHD-GIFs dataset. FCSN \cite{rochan2018video} and Video2GIF \cite{gygli2016video2gif} are two state-of-the-art generic highlight detection methods. A-VHD \cite{rochan2020adaptive} is the only one comparable method for personalized video highlight detection, to the best of our knowledge. SA-PR(*) stand for the different modification based on our method (Ablation experiments section). SA-PR(full) is our full method. }\label{tab:comparisons}
	\scalebox{1}{
	\begin{tabular}{c c}
        \hline
		\multirow{2}*{Method} &
		\multirow{2}*{mAP(\%)}\\

		~ & ~ \\
		\hline
		FCSN \cite{rochan2018video}& 15.15 \\
		Video2GIF \cite{gygli2016video2gif}& 14.55 \\
		A-VHD \cite{rochan2020adaptive}& 16.68 \\
        \hline
		SA-PR_{residual} & 16.69 \\
		SA-PR_{ranking} & 16.85 \\
		SA-PR_{CE} & 17.09 \\
		SA-PR_U & 17.57 \\
		SA-PR_G & 16.78 \\
		SA-PR_{h5} & 17.48 \\
		SA-PR_{full} & \textbf{18.66} \\ 
		
	\end{tabular}}
\end{table}
